MaZO: Masked Zeroth-Order Optimization for Multi-Task Fine-Tuning of Large Language Models

Large language models have demonstrated exceptional capabilities across diverse tasks, but their fine-tuning demands significant memory, posing challenges for resource-constrained environments. Zeroth-order (ZO) optimization provides a memory-efficient alternative by eliminating the need for backpropagation. However, ZO optimization suffers from high gradient variance, and prior research has largely focused on single-task learning, leaving its application to multi-task learning unexplored. Multi-task learning is crucial for leveraging shared knowledge across tasks to improve generalization, yet it introduces unique challenges under ZO settings, such as amplified gradient variance and collinearity. In this paper, we present MaZO, the first framework specifically designed for multi-task LLM fine-tuning under ZO optimization. MaZO tackles these challenges at the parameter level through two key innovations: a weight importance metric to identify critical parameters and a multi-task weight update mask to selectively update these parameters, reducing the dimensionality of the parameter space and mitigating task conflicts. Experiments demonstrate that MaZO achieves state-of-the-art performance, surpassing even multi-task learning methods designed for first-order optimization.

==> preliminary.tex <==






\section{Preliminaries}
\label{sec:preliminaries}
\subsection{Zeroth-order optimization}
Zeroth-order (ZO) optimization is a backpropagation-free method that estimates gradients using forward passes only. A common approach for gradient estimation in ZO optimization is the Simultaneous Perturbation Stochastic Approximation (SPSA) \citep{spall1992multivariate}, which serves as a randomized gradient estimator (RGE).

Consider a model with parameters $\theta \in \mathbb{R}^d$ and a loss function $\mathcal{L}(\theta)$. The Taylor expansion of the loss function around $\theta$ is given by:
\begin{equation}
\mathcal{L}(\theta + \delta \theta) = \left( \frac{\partial \mathcal{L}}{\partial \theta} \right)^\top \cdot \delta \theta + \frac{1}{2} \delta \theta^\top \cdot \mathbf{H} \cdot \delta \theta + \mathcal{O}(|\delta \theta|^3),
\end{equation}
where $H$ is the Hessian matrix.

To estimate the gradient, Zeroth-order optimization  replace $\delta \theta$ with $\epsilon \mathbf{z}$ and $-\epsilon \mathbf{z}$, where $\epsilon$ is a small scalar and $\mathbf{z} \sim \mathcal{N}(0, \bm{I}_d)$ is a random perturbation sampled from a normal distribution. Ignoring terms of third degree and higher, the estimated gradient is computed as:
\begin{align}
\widehat{\nabla} \mathcal{L}(\theta)
&= \frac{\mathcal{L}(\theta + \epsilon \mathbf{z}) - \mathcal{L}(\theta - \epsilon \mathbf{z})}{2 \epsilon} \mathbf{z} \\
&\approx \mathbf{z}\mathbf{z}^\top \nabla \mathcal{L}(\theta).
\end{align}

The expectation of the estimated gradient matches the true gradient:
\begin{align}
\mathbb{E}[\widehat{\nabla} \mathcal{L}(\theta)]
&= \mathbb{E}[\mathbf{z}\mathbf{z}^\top \nabla \mathcal{L}(\theta)] \\
&= \mathbb{E}[\mathbf{z}\mathbf{z}^\top] \nabla \mathcal{L}(\theta) \\
&= I_d \nabla \mathcal{L}(\theta) = \nabla \mathcal{L}(\theta),
\end{align}
where $I_d$ is the identity matrix.

During the training process, the random perturbation $\mathbf{z}$ is first sampled. Using forward and reverse perturbations, the losses $\mathcal{L}(\theta + \epsilon \mathbf{z})$ and $\mathcal{L}(\theta - \epsilon \mathbf{z})$ are computed, and the gradient estimate $\widehat{\nabla} \mathcal{L}(\theta)$ is obtained. Finally, the parameters are updated using zeroth-order stochastic gradient descent (ZO-SGD) as follows:
\begin{equation}
\theta = \theta - \eta \widehat{\nabla} \mathcal{L}(\theta),
\end{equation}
where $\eta$ is the learning rate.
\citet{malladi2023mezo} propose MeZO to regenerate the random perturbation $\mathbf{z}$ by random seed instead of storing $\mathbf{z}$ itself, which significantly reduce the memory consumption.


\subsection{Formulating Multi-task Learning}
\label{sec:reformmtl}

Multi-task learning (MTL) aims to improve generalization performance by jointly learning $N$ related tasks $\mathcal{T} = \{T_1, \dots, T_N\}$ through shared parameterization. Consider each task $T_i$ with dataset $\mathcal{D}_i = \{(x_i^{(j)}, y_i^{(j)})\}_{j=1}^{M_i}$, where $M_i$ denotes the sample size. The classical MTL objective minimizes the convex combination of task-specific losses:

\begin{align}
    & \mathcal{L}_{\text{MTL}}(\theta) = \sum_{t=1}^T w_t \mathcal{L}^t_{\text{STL}}(\theta),\\
    & \text{s.t.}\ \sum_{t=1}^T w_t = 1,\ w_t \geq 0
\end{align}

where $\mathcal{L}^t_{\text{STL}}(\theta) = \mathbb{E}_{(x,y)\sim\mathcal{D}_t}[\ell(f_\theta(x), y)]$ is the empirical risk for task $t$, and $\ell(\cdot)$ the loss function. Parameter updates follow:

\begin{equation}
    \theta \leftarrow \theta - \eta \nabla\mathcal{L}_{\text{MTL}}(\theta)
\end{equation}

\noindent\textbf{Challenge of Gradient Collinearity in ZO-MTL.} Under zeroth-order optimization, the task-specific gradient estimates exhibit fundamental collinearity. For task $t$, the ZO gradient estimator is:

\begin{equation}
    g^t_{\text{STL}} = \underbrace{\frac{\mathcal{L}^t_{\text{STL}}(\theta+\epsilon z) - \mathcal{L}^t_{\text{STL}}(\theta-\epsilon z)}{2\epsilon}}_{\text{scalar coefficient}} \cdot z
\end{equation}

where $z \sim \mathcal{N}(0,I_d)$ is the shared random perturbation. The MTL gradient aggregates these estimates:

\begin{align}
    g_{\text{MTL}} &= \sum_{t=1}^T w_t g^t_{\text{STL}} \\
    &= \underbrace{\left(\sum_{t=1}^T w_t \frac{\mathcal{L}^t_{\text{STL}}(\theta+\epsilon z) - \mathcal{L}^t_{\text{STL}}(\theta-\epsilon z)}{2\epsilon}\right)}_{\alpha(z)} \cdot z,
\end{align}

which is just a scaler times $z$.
This reveals the limitation: all task gradients align with $z$, losing directional diversity

Existing dynamic weighting schemes that manipulate $\{w_t\}$ only scale the scalar coefficient $\alpha(z)$, but cannot resolve directional conflicts. This necessitates a paradigm shift from loss weighting to parameter space interventions.

To overcome this limitation, we propose a novel multi-task learning approach that operates at the weight level rather than the loss scale or the gradient.

==> relatedwork.tex <==
\section{Related Work}

\zz{We need to merge Section 2 and Section 3.}
\subsection{Zeroth-Order Optimization}
Zeroth-order (ZO) optimizers utilize just two forward passes to estimate gradients without backpropagation, significantly lowering the GPU hours and memory usage compared to first-order (FO) optimizers \citep{tang2024private}. This offers a considerable advantage for fine-tuning large language models (LLMs), where the memory-intensive backpropagation process becomes a bottleneck as model sizes keep growing \citep{yang2024adazeta}.
Researchers have focused on improving the convergence rates and reducing gradient estimation variance of ZO optimization for LLM fine-tuning. Increasing batch size can diminish noise in ZO gradient estimation \citep{gautam2024variance}. Perturbing a subset of model parameters, either through random and sparse pruning masks or block-coordinate perturbations, also lowers gradient variance \citep{guo2024zeroth}. Additionally, some approaches try to reduce the number of trainable parameters through parameter-efficient fine-tuning (PEFT) techniques like tensorized adapters \citep{yang2024adazeta}.
Convergence theories for ZO optimization have been elaborated in both convex and non-convex settings. However, these convergence rates typically increase linearly with the number of trainable parameters 1. More recent work has focused on developing specialized ZO optimization methods with improved theoretical guarantees, such as the stagewise DP zeroth-order method (DP-ZOSO) \citep{liu2024differentially} and the Hessian-informed zeroth-order optimizer (HiZOO) \citep{zhao2024second}.

\subsection{Multi-task Learning under First-Order Setting}

Multi-task learning (MTL) has been widely studied in the context of deep learning, where the goal is to leverage shared representations across multiple related tasks to improve the overall performance. Several works have explored first-order optimization methods for MTL.
One line of research focuses on using scalarization techniques to combine the losses of multiple tasks into a single objective function, which can then be optimized using standard first-order methods like stochastic gradient descent (SGD) \citep{hu2024revisiting}. However, these approaches have been shown to struggle in reaching the Pareto frontier, which represents the optimal trade-off between the different task objectives .
To address this issue, some studies have proposed using uncertainty weighting to balance the losses of different tasks during training \citep{xin2022current}. This approach aims to automatically adjust the importance of each task based on the model's confidence, rather than relying on manual task weighting.
Another direction is to leverage the task relationships or affinities to guide the optimization process. For example, \citet{li2024scalable} introduced a gradient-based estimation method to approximate the fine-tuning performance of different task subsets, allowing for efficient subset selection during multi-task learning \citep{samant2022framework}. This approach can be particularly useful for large-scale language model fine-tuning, where choosing the right auxiliary tasks is crucial.

